Probabilistically Robust Watermarking of Neural Networks

As deep learning (DL) models are widely and effectively used in Machine Learning as a Service (MLaaS) platforms, there is a rapidly growing interest in DL watermarking techniques that can be used to confirm the ownership of a particular model. Unfortunately, these methods usually produce watermarks susceptible to model stealing attacks. In our research, we introduce a novel trigger set-based watermarking approach that demonstrates resilience against functionality stealing attacks, particularly those involving extraction and distillation. Our approach does not require additional model training and can be applied to any model architecture. The key idea of our method is to compute the trigger set, which is transferable between the source model and the set of proxy models with a high probability. In our experimental study, we show that if the probability of the set being transferable is reasonably high, it can be effectively used for ownership verification of the stolen model. We evaluate our method on multiple benchmarks and show that our approach outperforms current state-of-the-art watermarking techniques in all considered experimental setups.

==> FormattingGuidelines-IJCAI-24/extra_not_used_related.tex <==
The process of watermarking deep neural networks serves the purpose of safeguarding intellectual property by encoding a distinctive pattern and employing it for the purpose of asserting ownership \cite{ahmed:ieee-steganography}. Generally, a model stealing attack involves the illicit acquisition of a target model $f$ by leveraging black-box access. This means that the attacker interacts with the model by making queries through a predefined interface. By making such queries to $f$ an attacker can gather labels for previously unlabeled data samples $\mathcal{D}$ from the distribution $\mathcal{D}$. Subsequently, armed with both $\mathcal{D'}$ and the corresponding labels derived from the original model, the attacker can proceed to train a surrogate model $f*$ that replicates the functionality of the original model\cite{carlini:2020cryptanalytic}.  The objectives for ensuring security can be delineated through criteria that define the efficacy of a watermarking system. Today, the watermarking techniques include embedding watermarks into model parameters\cite{Wang:2020Watermarking}, employing pre-defined inputs as triggers \cite{lemerrer:stiching}. The latter 
is reported as featuring limited integrity, as in today's landscape, adversarial retraining is widely employed to enhance model robustness \cite{Namba.2019Robust}.

% Types of settings
The type of access required to perform watermark verification on a model depends on the embedding method used to insert the watermark. There are two primary scenarios for watermark verification: white-box and black-box.
In a white-box scenario, a legitimate model owner must have access to the model's parameters to check for the watermark in potentially stolen copies of the model. This becomes necessary when the watermark is embedded solely within the model parameters and doesn't manifest in the model's behavior. However, in many cases, assuming white-box access for verification is not practical. A more realistic approach is the black-box access scenario, where a legitimate model owner can interact with the potentially stolen model only through a predefined query interface. Using this interface, the model owner can query (parts of) the watermark trigger and identify a stolen instance of the model based on its prediction behavior on these data points.

When choosing an appropriate watermarking method, it's crucial to consider the access scenario for verification. This is because a watermark that relies on the model owner having access to the model parameters for verification may not be effective in a scenario where the attacker deploys the stolen model in a black-box setting.
% Types of settings

% Requirements
In the context of watermarking, security objectives can be defined through specific requirements for an effective watermarking system. Over recent years, various parties have articulated such requirements, as demonstrated by sources like \cite{Uchida.2017Embedding,Adi.2018Turning,Chen.2019DeepMarks}. 

It's worth mentioning that implementing all of these requirements simultaneously may not be feasible, as they can potentially conflict with one another. Consider the example of "reliability" and "integrity." To ensure a watermark's reliability, the verification process should be highly sensitive and indicate ownership even in cases of uncertainty. A watermarking scheme where verification always signals ownership for every tested model would be considered highly reliable, as it would detect every stolen model instance. However, such a scheme would also have a very high rate of false alarms, wrongly accusing many honest parties of theft, which would compromise its integrity.
% Requirements


In \cite{jia:mmt}, 
and recently, in \cite{kim2023margin}
a new type of stealing attacks with the margin-based technique that improves the prediction ability of the attack model is proposed. Recent techniques include targeted DNN-fingerprint removal \cite{hongwei:removal}.





%----------

\subsection{Drawbacks discussion (remove in final submission)}

In trigger dataset-based watermarking approaches, watermark detection depends on the model's responses to queries from the trigger dataset. If the model's predictions align with the original labels of the trigger dataset beyond a specified threshold, it suggests the presence of the watermark. However, setting an appropriate threshold for identifying a stolen model requires careful tuning. Setting it too high may make slight modifications in a stolen model sufficient to evade watermark detection, compromising reliability. Conversely, setting it too low might lead to erroneous identification of different models as stolen instances, affecting integrity. Thus, the choice of the threshold involves a trade-off between reliability and integrity.

In addition to the threshold challenge, \cite{Hitaj.2018Have} highlighted a drawback for public verification scenarios. They argued that after running the verification algorithm against a stolen model, the attacker gains access to the trigger dataset, allowing fine-tuning of the model to remove the watermark. This limitation arises from the maximum number of backdoors that can be embedded in a neural network. Approaches requiring fewer queries, such as \cite{jia2021entangled}, may allow for more independent watermark verifications with the same model capacity.

Furthermore, watermarking schemes that embed watermarks into machine learning model parameters without precautions not only leave a detectable trace in the model but often rely on white-box access for verification. While white-box access may be feasible in some scenarios, assuming black-box access is often more realistic. Therefore, such schemes may be suitable for specific applications only.

Additionally, watermarking schemes lacking a verifiable link between the watermark and the legitimate model owner enable attackers to forge the watermark. This issue also applies to schemes using non-specific data points as trigger data (e.g., \cite{Adi.2018Turning,Guo.2018Watermarking}. Approaches preventing already marked models from being marked again, like \cite{Li.2019Piracy}, can mitigate this threat.

Finally, adversarial examples used for watermarking or fingerprinting, due to their instability, potential vulnerability to fine-tuning, and transferability, may violate watermark integrity. For instance, \cite{Namba.2019Robust} point out that adjusting the model's decision boundary based on adversarial examples, as seen in \cite{lemerrer:stiching}, may not fit the integrity requirement, as it resembles the effects of adversarial retraining, a method used to enhance the robustness of machine learning models.

The primary limitation of watermarking is its passive nature, as it can only detect theft after the fact without preventing it. Some research aims to issue security warnings when an ML model begins revealing enough information for potential attackers to extract its functionality \cite{Kesarwani.2018Model}. Additional efforts explore the development of theft-resistant models, such as those providing only hard labels without probabilities, perturbing prediction outputs \cite{Orekondy.2019Prediction}, or designing highly sensitive networks that deter attackers from stealing and adapting them \cite{Szentannai.2019MimosaNet}. Future work could investigate integrating watermarking into these active defense strategies against model theft.

Most existing watermarking schemes are designed for image data, with only a few exceptions, like \cite{jia2021entangled,Behzadan.2019Sequential,ong2021protecting,lim2020protect}, demonstrating applicability to other data types. Future research should explore the generality and universal applicability of these schemes, potentially requiring adaptation or extension.

Furthermore, most watermarking approaches primarily target classification tasks, with limited exploration in other ML domains, such as reinforcement learning \cite{Behzadan.2019Sequential}, data generation using GANs \cite{ong2021protecting}, or image captioning \cite{lim2020protect}. Thus, there is a promising challenge in developing watermarking schemes for various ML applications.

Additionally, existing watermarking schemes have mainly been applied and evaluated on small research datasets like MNIST \cite{LeCun.2010MNIST}. The scalability of these approaches remains an open question. Approaches requiring training with double the initial data might not be feasible in all scenarios. Therefore, future work should assess the practical applicability of existing watermarking schemes on larger real-world datasets and examine whether the properties observed on research datasets (training efficiency, reasonable trigger dataset size, integrity, etc.) hold true.

In contrast to earlier watermarking and ownership verification techniques, our method relies on probabilistic approach to improve the resilience of watermarking methods based on trigger sets against stealing attacks. Our approach is versatile and can be applied to enhance the resilience of any watermarking technique that relies on trigger sets, making it universally applicable and robust to functionality stealing methods.

% This allows us to differentiate between a model trained with the trigger set and one trained without it.

% \subsection{DNN Watermarking}

% \subsection{Trigger set approaches}
% In summary, traditional watermarking algorithms are good in particular cases but lame given real-world settings. 

==> FormattingGuidelines-IJCAI-24/table0.tex <==
\begin{table*}
    \centering
    \caption{Accuracy taable for ResNet-34.}
    \label{tab:accuracy}
    \begin{tabular}{llllllllll}
    \hline
        \textbf{Train Dataset } & \textbf{Cifar10} & \textbf{Cifar10} & \textbf{Cifar10} & \textbf{Cifar10} & \textbf{Cifar10} & \textbf{Cifar100} & \textbf{Cifar100} & \textbf{Cifar100} & \textbf{Cifar10} \\ \hline
        \textbf{Train Acc } & 0,971 & 0,971 & 0,971 & 0,971 & 0,971 & 0,97 & 0,97 & 0,97 & 0,971 \\ 
        \textbf{Test Acc } & 0,9 & 0,9 & 0,9 & 0,9 & 0,9 & 0,667 & 0,667 & 0,667 & 0,9 \\ \hline
    \end{tabular}
\end{table*}
